Topologically Massive Yang-Mills Theory and Link Invariants (Thesis)

In this thesis, topologically massive Yang-Mills theory is studied in the framework of geometric quantization. This theory has a mass gap that is proportional to the topological mass $m$. Thus, Yang-Mills contribution decays exponentially at very large distances compared to $1/m$, leaving a pure Chern-Simons theory with level number $k$. The focus of this research is the $near$ Chern-Simons limit of the theory, where the distance is large enough to give an almost topological theory, with a small contribution from the Yang-Mills term. It is shown that this almost topological theory consists of two copies of Chern-Simons with level number $k/2$, very similar to the Chern-Simons splitting of topologically massive AdS gravity model. As $m$ approaches to infinity, the split parts add up to give the original Chern-Simons term with level $k$. Also, gauge invariance of the split Chern-Simons theories is discussed for odd values of $k$. Furthermore, a relation between the observables of topologically massive Yang-Mills theory and Chern-Simons theory is obtained. It is shown that one of the two split Chern-Simons pieces is associated with Wilson loops while the other with 't Hooft loops. This allows one to use skein relations to calculate topologically massive Yang-Mills theory observables in the near Chern-Simons limit. Finally, motivated with the topologically massive AdS gravity model, Chern-Simons splitting concept is extended to pure Yang-Mills theory at large distances. It is shown that pure Yang-Mills theory acts like two Chern-Simons theories with level numbers $k/2$ and $-k/2$ at large scales. At very large scales, these two terms cancel to make the theory trivial, as required by the existence of a mass gap.

==> Prelude/dedication.tex <==
To my parents:\\
Pakize and Yadigar Yildirim

==> Prelude/publicAbstract.tex <==
Yang-Mills theory is a very important part of the Standard Model of particle physics. Despite its success in explaining the high-energy physics, its mathematical behavior is very difficult to understand at low energies. This difficulty gave birth to a simplified program, pioneered by Feynman(1981). Feynman suggested that, in order to understand the qualitative behavior of the theory, one can study it in two space and one time dimensions instead of the actual 3+1 dimensional case. 

There is another important 2+1 dimensional theory in mathematical physics, called the Chern-Simons theory. This theory is related to knot theory, which was shown by Witten(1989). Chern-Simons theory is very useful in condensed matter physics, especially in the fractional quantum hall effect phenomena. 

This thesis studies a mixture of these two 2+1 dimensional theories, called the "Topologically Massive Yang-Mills theory". Unlike Chern-Simons theory, Yang-Mills theory is not directly related to knot theory. But Topologically Massive Yang-Mills theory has an interesting low energy behavior that allows one to use knot theory. This relation is the main result of this thesis and it provides a nice extension to the relations between field theories and knot theory. The results of this thesis can be used in some condensed matter theory applications and also, it may provide valuable insight in studying 2+1 dimensional particle physics.

==> Prelude/thesisAbstract.tex <==
In this thesis, topologically massive Yang-Mills theory is studied in the framework of geometric quantization. This theory has a mass gap that is proportional to the topological mass $m$. Thus, Yang-Mills contribution decays exponentially at very large distances compared to $1/m$, leaving a pure Chern-Simons theory with level number $k$. The focus of this research is the \emph{near} Chern-Simons limit of the theory, where the distance is large enough to give an almost topological theory, with a small contribution from the Yang-Mills term. It is shown that this almost topological theory consists of two copies of Chern-Simons with level number $k/2$, very similar to the Chern-Simons splitting of topologically massive AdS gravity model. As $m$ approaches to infinity, the split parts add up to give the original Chern-Simons term with level $k$. Also, gauge invariance of the split Chern-Simons theories is discussed for odd values of $k$. Furthermore, a relation between the observables of topologically massive Yang-Mills theory and Chern-Simons theory is obtained. It is shown that one of the two split Chern-Simons pieces is associated with Wilson loops while the other with 't Hooft loops. This allows one to use skein relations to calculate topologically massive Yang-Mills theory observables in the near Chern-Simons limit. Finally, motivated with the topologically massive AdS gravity model, Chern-Simons splitting concept is extended to pure Yang-Mills theory at large distances. It is shown that pure Yang-Mills theory acts like two Chern-Simons theories with level numbers $k/2$ and $-k/2$ at large scales. At very large scales, these two terms cancel to make the theory trivial, as required by the existence of a mass gap.

==> Prelude/thesisAck.tex <==
The idea of studying Chern-Simons link invariants modified with the presence of a small Yang-Mills term was proposed by my PhD advisor Prof. Vincent Rodgers and Prof. Parameswaran Nair. I am truly grateful and honored to work with them. I cannot thank enough for the time and effort they spent to help me. Especially, I want to thank my advisor Prof. Rodgers for taking me under his guidance, providing a great working environment, being a great mentor and a friend. 

I thank the members of my thesis committee: Profs. Charles Frohman, Craig Pryor, Wayne Polyzou and Mary Hall Reno for their time, help and support. Especially to Prof. Charles Frohman for his encouragement and his help on knot theory. I thank professors Yannick Meurice, Yasar Onel, Sujeev Wickramasekara, Craig Kletzing, Maxim Khodas for their support and encouragement. I am thankful to Prof. Brian C. Hall for his time, support and help on geometric quantization. I also would like to acknowledge helpful comments from Profs. Edward Witten, Chris Baesley and Dr. Tudor Dimofte.

I am grateful to the current and previous members of the Diffeomorphism and Geometry Research Group: Dr. Brad Button, Chris Doran, Delalcan Kilic, Dr. Xiaolong Liu, Dr. Leo Rodriguez, Dr. Kory Stiffler and Catherine Whiting for their support and true friendship. Leo Rodriguez helped me so much, he was almost like a co-advisor to me during my first years in Iowa. Brad Button's support and friendship helped me go through some of the most difficult stages in graduate school. I thank Marc Herrmann for very helpful discussions and his support. I also would like to thank Cuneyt Sahin for his endless support and being a true friend.  

I would like to thank my students Suzanne Carter, Wade Bloomquist and Hart Goldman for their interest in this research and checking some of my calculations. 

I would like to thank the Physics and Astronomy department staff Debbie Foreman, Heather Mineart, Jeanne Mullen, Chris Stevens, Ron Vogel and Aaron Votroubek for being so helpful throughout my graduate school years.

I would like to thank the Beyond Center for Fundamental Concepts in Science at Arizona State University for their hospitality, where I wrote the final sections of this thesis. Especially Profs. Maulik Parikh and Tanmay Vachaspati, Dr. Eray Sabancilar and Subir Sabharwal for their support and helpful comments.

Finally, I would like to thank my family. Without their love and support, it would be impossible for me to accomplish anything. I cannot thank my parents Pakize and Yadigar Yildirim enough for their support and sacrifices. I am grateful to my brother Bora Yildirim for his support and encouragement.

This work was partially supported by National Science Foundation grant NSF1067889.

